The reverse mathematics of Cousin's lemma

Cousin's lemma is a compactness principle that naturally arises when studying the gauge integral, a generalisation of the Lebesgue integral. We study the axiomatic strength of Cousin's lemma for various classes of functions, using Friedman and Simpson's reverse mathematics in second-order arithmetic. We prove that, over $\mathsf{RCA}_0$: (i) Cousin's lemma for continuous functions is equivalent to the system $\mathsf{WKL}_0$; (ii) Cousin's lemma for Baire 1 functions is at least as strong as $\mathsf{ACA}_0$; (iii) Cousin's lemma for Baire 2 functions is at least as strong as $\mathsf{ATR}_0$.

==> acknowledge.tex <==
\chapter*{Acknowledgments}\label{C:ack} 

I must, of course, thank my supervisors, Rod Downey and Noam Greenberg, for introducing me to the weird and wonderful world of reverse mathematics

Rod, Noam

I owe a great debt to Martino Lupini for his <> support throughout the years
Martino
family
Other hons students \& grads
uke club

==> chapter.tex <==
\chapter{Chapter}
...
